Branch-and-Price for the Stochastic TSP with Generalized Latency

Motivated by the tactical planning level of demand adaptive public transportation systems, we present the stochastic symmetric traveling salesman problem with generalized latency (STSP-GL), a stochastic extension to the symmetric traveling salesman problem with generalized latency (TSP-GL). The STSP-GL aims to choose a subset of nodes of an undirected graph and determines a Hamiltonian tour amongst those nodes, minimizing an objective function that is a weighted combination of route design and passenger routing costs. These nodes are selected to ensure that a predefined percentage of uncertain passenger demand is served with a given probability. We formulate the STSP-GL as a stochastic program and propose a branch-and-price algorithm for solving its deterministic equivalent. We also develop a local search approach with which we improve the performance of the B&P approach. We assess the efficiency of the proposed methods on a set of instances from the literature. We demonstrate that the proposed methods outperform a known benchmark, improving upper bounds by up to 85% and lower bounds by up to 55%. Finally, we show that solutions of the stochastic model are both more cost-effective and robust than those of the deterministic model.

==> contents/conclusions.tex <==
\section{Conclusion}
\label{sec: conclusion}

With this work, we introduced an algorithmic framework to determine the system optimum of an intermodal transportation system. To do so, we modeled a transportation system as a partially time-expanded digraph, which implicitly encodes problem specific constraints related to the intermodality of the problem. This allowed us to find the intermodal transportation system's optimum by solving a standard integer minimum-cost multi-commodity flow problem. We solved this problem with a column generation based price-and-branch approach, for which we introduced a pricing filter to reduce the number of solved pricing problems. Furthermore, we proposed a distance approximation to utilize the $A^*$ algorithm to solve the pricing problems more efficiently. We applied our methodology to a real-world case study for the city of Munich. Our results show that our pricing filter reduces the computation time of our algorithm by up to 60\% and the application of the $A^*$-based pricing algorithm additionally reduces it by up to 90\%. Our algorithm is able to solve unimodal instances with 23,688 trips in 11 minutes and intermodal instances with 56,295 trips in 48 minutes, whereas straightforward MIP models fail to solve instances with more than a few hundred trips.

==> resources/commands.tex <==
%% additional user defined commands

